Exploring the Design Space of Visual Context Representation in Video MLLMs

Video Multimodal Large Language Models (MLLMs) have shown remarkable capability of understanding the video semantics on various downstream tasks. Despite the advancements, there is still a lack of systematic research on visual context representation, which refers to the scheme to select frames from a video and further select the tokens from a frame. In this paper, we explore the design space for visual context representation, and aim to improve the performance of video MLLMs by finding more effective representation schemes. Firstly, we formulate the task of visual context representation as a constrained optimization problem, and model the language modeling loss as a function of the number of frames and the number of embeddings (or tokens) per frame, given the maximum visual context window size. Then, we explore the scaling effects in frame selection and token selection respectively, and fit the corresponding function curve by conducting extensive empirical experiments. We examine the effectiveness of typical selection strategies and present empirical findings to determine the two factors. Furthermore, we study the joint effect of frame selection and token selection, and derive the optimal formula for determining the two factors. We demonstrate that the derived optimal settings show alignment with the best-performed results of empirical experiments. Our code and model are available at: https://github.com/RUCAIBox/Opt-Visor.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/old_experiment.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{Scaling of visual tokens per frame}
\label{sec:scaling_tokens}

% \paragraph{Scaling the visual tokens improves performance in general, but the gains diminish after a certain point for some benchmarks.}
We fix the number of frames and train a series of models with the number of visual tokens ranging from 1 to 196, using the method introduced in Section~\ref{sec:vary_tokens}. Then we propose the following function to fit the scaling law of visual tokens:
\begin{equation}
    \mathcal{L}(M) = E_M + \left(\frac{M_0}{M}\right)^{a_M}
\end{equation}

We fit the losses with the number of visual tokens $T$ using the scipy curvefit function, obtaining $E_m=0.57, M_0=0.01, a_M=0.39$, with $R^2=0.987$ indicating a good fit.

As for the zero-shot accuracy on the evaluation benchmarks, Table~\ref{tab:compressing_token_result} and Table~\ref{tab:sampling_token_result} show that all benchmarks show consistent improvements as the number of tokens increases. For instance, VNBench improves from 18.44 to 31.56, and VideoMME (wo-subs) increases from 41.33 to 53.56 as the number of tokens per frame rises from 1 to 196. However, there is a threshold beyond which further increasing the number of visual tokens yields only marginal gains or even slight drops. For example, increasing the tokens from 81 to 196 results in just a 0.11 improvement on VideoMME (w-subs). Notably, increasing the tokens from 81 to 196 even causes a performance drop on the MLVU benchmark. In addition, Figure~\ref{fig:VideoMME_acc_token} shows the performance across different subsets of the VideoMME benchmark. We observe that increasing the token count from 1 to 16 results in significant improvements, but further increases lead to only minor fluctuations or marginal gains. Specifically, the improvement from 81 to 196 tokens is minimal. These findings suggest that while increasing the number of tokens is generally beneficial, an excessive number can result in diminishing returns, emphasizing the need to find a ``golden point'' that balances performance with a moderate token count.

\setlength{\tabcolsep}{5.5pt} % 减小列间距
\begin{table}[h]
\caption{Experimental results under different number of visual tokens per frame, with the compressing-based method.}
    \small
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
 \# Frames&\makecell[c]{\# Tokens/\\Frames}&    \makecell[c]{\# Total\\Tokens}&\makecell[c]{Event-\\Bench}&  \makecell[c]{VNBench}& \makecell[c]{MLVU}&  \makecell[c]{LongVideo-\\Bench} &\makecell[c]{VideoMME\\wo/w-subs}   &Avg.\\
    \midrule
         32& 1&32 & 18.67& 18.44& 49.45& 39.88&41.33/49.15 &36.15\\
         32& 4&128 & 24.33& 27.04& 52.77& 43.44&46.11/55.93 &41.60\\
         32&9&    288&22.33&  27.41&  53.83&  45.11&47.78/55.41 &41.98\\
         32&16&   512&20.33& 28.96& 55.04&  46.32&49.85/58.15 &43.11\\
         32&25&   800&23.00& 28.67& 54.21&  46.02&49.85/58.11 &43.31\\
         32&36&    1152&\underline{27.33}&  \underline{30.00}&  53.73&  48.45&50.33/58.74 &\underline{44.76}\\
         32&49&    1568&21.33&  29.93&  54.84&  47.16&49.96/58.37 &43.60\\
         32&81&    2592&23.33&  27.33&  \textbf{57.59}&  \underline{48.60}&\underline{52.00}/\underline{59.37} &44.70\\
         32&196&    6272&\textbf{29.00}&  \textbf{31.56}&  \underline{56.81}&  \textbf{52.24}&\textbf{53.56/59.48} &\textbf{47.11}\\
    \bottomrule
    \end{tabular}
    \label{tab:compressing_token_result}
\end{table}

\setlength{\tabcolsep}{6pt} % 减小列间距
\begin{table}[h]
\caption{Experimental results under different number of visual tokens per frame, with the sampling-based method.}
    \small
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
 \# Frames&\makecell[c]{\# Tokens/\\Frames}&    \makecell[c]{\# Total\\Tokens}&\makecell[c]{Event-\\Bench}&  \makecell[c]{VNBench}& \makecell[c]{MLVU}&  \makecell[c]{LongVideo-\\Bench} &\makecell[c]{VideoMME\\wo/w-subs}   &Avg.\\
    \midrule
         32& 1&32 & 21.67& 14.96& 48.67& 40.56&42.48/52.04&36.73\\
         32& 4&128 & 23.33& 21.11& 50.72& 44.88&45.44/54.81&40.05\\
         32&9&    288&25.33&  24.15&  52.42&  43.82&45.85/54.67&41.04\\
         32&16&   512&23.00& 27.85& 52.29&  46.70&49.22/57.11&42.20\\
         32&25&   800&22.33& 26.22& 55.18&  47.08&50.44/58.26&43.25\\
         32&36&    1152&20.33&  29.48&  56.05&  47.76&50.07/58.04&43.62\\
         32&49&    1568&23.33&  28.52&  55.41&  48.90&51.30/59.74&44.53\\
         32&81&    2592&24.00&  29.41&  55.12&  48.90&50.04/57.30&44.13\\
         32&196&    6272&26.00&  27.78&  56.53&  47.69&48.63/55.59&43.70\\
    \bottomrule
    \end{tabular}
    \label{tab:sampling_token_result}
\end{table}

\begin{figure}[h]
  \centering
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/VideoMME_acc_token.pdf}
    \caption{The relationship between the number of tokens per frame during model training and the test accuracy.}
    \label{fig:VideoMME_acc_token}
  \end{minipage}
  \hspace{0.05\linewidth}
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/VideoMME_acc_frame.pdf}
	  \caption{The relationship between the number of frames during model training and the test accuracy.}
	  \label{fig:VideoMME_acc_frame}
  \end{minipage}
\end{figure}


\subsection{Scaling of frames}
\label{sec:scaling_frames}
Since the limited computation budget does not allow us to keep all the visual tokens per frame and scale the number of frames from 8 to 128, we first reduce the number of tokens in a frame using the method in \ref{sec:vary_tokens} and keep it fixed, then scale the number of frames to conduct the experiment. According to the result in Table~\ref{tab:compressing_token_result}, setting $p=4$ reduces the number of visual tokens per frame to 93\% of the original one, and maintains the performance on most benchmarks. As a result, we adopt $4\times 4$ MeanPooling to keep 49 tokens per frame and set $T=\{1,8,16,32,64,96,128\}$ to explore the scaling of the number of frames. We train 7 video MLLMs under these settings, with the results of each benchmark illustrated in Table~\ref{tab:sampling_frame_result}. We could obtain the following conclusion:

\paragraph{Scaling the number of frames improves performance on all benchmarks, although the improvement varies slightly across benchmarks.} The results in Table \ref{tab:sampling_frame_result} demonstrate a clear trend where increasing the number of frames consistently improves performance across all benchmarks. As the number of frames scales from 8 to 128, significant gains are observed, with the most substantial improvements seen at 128 frames. Notably, the impact of scaling frames varies slightly across benchmarks: for example, VNBench and MLVU show more pronounced improvement (from 15.70 to 39.70 and from 46.30 to 61.44) compared to EventBench and LongVideoBench, which see a more modest increase (from 21.67 to 25.67 and from 44.73 to 51.40). This suggests that certain tasks benefit more from additional temporal context (\eg the Needle-In-the-Haystack-Search~(NIAH) task in VNBench and MLVU), while others display more conservative gains (\eg the episodic reasoning task in Event-Bench and LongVideoBench). Overall, increasing the number of frames enhances model performance, though the extent of improvement depends on the specific characteristics of each benchmark. Figure~\ref{fig:VideoMME_acc_frame} illustrates the performance across different subsets of the VideoMME benchmark for models trained with varying numbers of frames. As the number of frames increases, the model consistently improves on videos of different lengths, with no clear saturation point even at 128 frames—exceeding the limits of most video MLLMs. Compared to scaling the number of tokens per frame (Figure~\ref{fig:VideoMME_acc_token}), increasing the number of frames proves to be more beneficial for overall performance.

\paragraph{Scaling the number of frames compensates for reducing the number of tokens per frame.} The results in Table~\ref{tab:compressing_token_result} show that reducing the number of visual tokens per frame from 196 to 49 leads to a performance drop across all benchmarks. However, increasing the number of frames simultaneously can mitigate this drop. For instance, comparing the last rows of Table~\ref{tab:compressing_token_result} and Table~\ref{tab:sampling_frame_result}, both setups use a total of 6272 visual tokens, but one utilizes 32 frames with 196 tokens per frame, while the other employs 128 frames with 49 tokens per frame. The model trained on more frames and fewer tokens per frame performs significantly better overall, except for LongVideoBench, where the configuration with fewer frames and more tokens per frame shows a slight advantage (52.24 vs. 51.40). These results suggest that, when constrained by the same total number of tokens, increasing the number of frames while decreasing the tokens per frame enhances performance on most benchmarks and maintains competitive results on others.

\setlength{\tabcolsep}{6pt} % 减小列间距
\begin{table}[h]
\caption{Experimental results under different number of frames, with the compressing-based method. * For the model trained with 128 frames, since $T_{\text{max}} = T = 128$ in this setting, the temporal pooling kernel size is $l = \lceil \frac{128}{128} \rceil = 1$, resulting in the same outcome as the sampling-based method.}
    \small
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
\makecell[l]{\# Frames} & \makecell[c]{\#Tokens/\\Frames}&    \makecell[l]{\# Total\\Tokens}&\makecell[c]{Event-\\Bench}&  \makecell[c]{VNBench}& \makecell[c]{MLVU}&  \makecell[c]{LongVideo\\Bench} &\makecell[c]{VideoMME\\wo/w-subs}  &Avg.\\
    \midrule
        8 &49&    392 &25.67&  20.89&  53.04&  46.32& 50.48/57.41&42.30\\
        16 &49&   784 &\underline{27.00}& 27.04& 55.77&  48.07& 50.44/58.30&44.44\\
        32 &49&   1568 &25.33& 29.78& 59.37&  48.52& \underline{53.81}/\underline{60.93}&46.29\\
        48&49&   2352&24.33& 37.41& 59.31&  47.61& 52.07/59.81&46.76\\
        64 &49&    3136 &\textbf{29.00}&  36.3&  \underline{61.03}&  
        47.61& 53.70/60.56&\underline{48.03}\\
        96& 49& 4704& \underline{27.00}& \underline{38.22}& 59.35& \underline{49.13}& 53.67/60.26&47.94\\
        128$^*$ &49&    6272&25.67&  \textbf{39.70}&  \textbf{61.44}&  \textbf{51.40}& \textbf{56.11}/\textbf{61.63} &\textbf{49.33}\\
    \bottomrule
    \end{tabular}
    \label{tab:compressing_frame_result}
\end{table}

\setlength{\tabcolsep}{6pt} % 减小列间距
\begin{table}[h]
\caption{Experimental results under different number of frames, with the sampling-based method.}
    \small
    \centering
    \begin{tabular}{ccccccccc}
    \toprule
\makecell[l]{\# Frames} & \makecell[c]{\#Tokens/\\Frames}&    \makecell[l]{\# Total\\Tokens}&\makecell[c]{Event-\\Bench}&  \makecell[c]{VNBench}& \makecell[c]{MLVU}&  \makecell[c]{LongVideo\\Bench} &\makecell[c]{VideoMME\\wo/w-subs}  &Avg.\\
    \midrule
        8 &49&    392 &21.67&  15.70&  46.30&  44.73&44.85/52.74 &37.67\\
        16 &49&   784 &22.67& 23.33& 52.53&  46.78&49.74/57.59 &42.11\\
        32 &49&   1568 &21.33& 29.93& 54.84&  47.16&49.96/58.37 &43.60\\
        48&49&   2352&22.67& 34.15& 56.22&  \underline{48.75}&52.81/59.11 &45.62\\
        64 &49&    3136 &25.33&  32.59&  57.23&  
        47.08&52.59/58.93 &45.63\\
        96& 49& 4704& \textbf{26.67}& \underline{37.26}& \underline{60.97}& 48.60&\underline{53.26}/\underline{60.85} &\underline{47.94}\\
        128 &49&    6272&\underline{25.67}&  \textbf{39.70}&  \textbf{61.44}&  \textbf{51.40}&\textbf{56.11}/\textbf{61.63} &\textbf{49.33}\\
    \bottomrule
    \end{tabular}
    \label{tab:sampling_frame_result}
\end{table}



% \begin{table}
%     \centering
%     \caption{Results on VideoMME different duration split.}
%     \begin{tabular}{ccccc}
%     \toprule
%            \# Frames&  Short&  Medium&  Long& Overall\\
%     \midrule
%            8&  54.1&  41.4&  39.0& 44.9\\
%            16&  60.2&  47.8&  41.2& 49.7\\
%            32&  61.3&  46.8&  41.8& 50.0\\
%            48&  64.3&  50.7&  43.4& 52.8\\
%             64& 65.1& 50.8& 41.9&52.6\\
%             96&  64.6&  50.8&  44.4& 53.3\\
%             128& 67.7& 54.6& 46.1&56.1\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:videomme_result}
% \end{table}

% \begin{table}
%     \centering
%     \caption{Results on VideoMME different duration split.}
%     \begin{tabular}{ccccc}
%     \toprule
%            Tokens&  Short&  Medium&  Long& Overall\\
%     \midrule
%            1&  48.3&  40.0&  35.7& 41.3\\
%            4&  54.3&  45.3&  38.7& 46.1\\
%            9&  56.7&  46.8&  39.9& 47.8\\
%            16&  59.8&  47.2&  42.6& 49.9\\
%             25& 60.9& 46.4& 42.2&49.9\\
%             36&  61.6&  47.8&  41.7& 50.3\\
%             49& 61.3& 46.8& 41.8&50.0\\
%  81& 63.8& 49.4& 42.8&52.0\\
%  196& 64.6& 51.9& 44.2&53.6\\
%  \bottomrule
%     \end{tabular}
%     \label{tab:videomme_result}
% \end{table}

% \begin{table}
%     \caption{Caption}
%     \centering
%     \begin{tabular}{ccccc}
%     \toprule
%            &  \multicolumn{4}{c}{Video Duration}\\
%            \# Frames&  (8,15]&  (15,60]&  (180,600]& (900,3600]\\
%     \midrule
%          8& 53.44&56.98&42.61&39.49\\
%           16& 54.50& 61.05& 46.80& 39.67\\
%           32& 56.08& 60.47& 44.09& 42.21\\
%            64&  51.85&  61.63&  45.57& 42.03\\
%            128&  59.26&  62.79&  51.72& 44.93\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}


\subsection{Trade-off between tokens and frames}
According to the conclusion in Section~\ref{sec:scaling_tokens} and Section~\ref{sec:scaling_frames}, where scaling both the visual tokens and the frames can improve performance, and increasing the number of frames could compensate for the reduction of visual tokens, it is natural to ask: \emph{how to balance the number of visual tokens and frames under the constrain of context window size of LLM?} 

To answer this question, we measure the scaling law along the token and frame axes. Specifically, we set the number of visual tokens as $\{25,49,81\}$, and set the number of frames as $\{48,64,80\}$, train $3\times 3=9$ models in total, and calculate the average loss of the last 100 steps. Then we fit the losses with token count $M$ and frame count $T$ following \citet{hoffmann2022training}:

\begin{equation}
    L(M,T)=C_M\times M^{-\alpha}+C_T\times T^{-\beta}+L_0
\end{equation}

We obtain $C_M=, \alpha=, C_T=, \beta=, L_0=$, where $R^2=$ indicates a good fit.

To make a direct application to the model development and an obvious comparison, we constrain the context window size of LLM as 8K, and set the visual context window size as 6K, obtaining the following configurations: $\{8 \text{frame}\times 729 \text{token}\}, \{30 \text{frame}\times 196 \text{token}\}, \{72 \text{frame}\times 81 \text{token}\}, \{120 \text{frame}\times 49 \text{token}\}, \{162 \text{frame}\times 36 \text{token}\}$\footnote{Some groups result in 5832 tokens while ther others result in 5880 tokens in total, this is because the number of visual tokens produced by MeanPooling without overlapping must be the square of integer (\eg, $1^2, 2^2, 3^2, \cdots$). Considering the large number of tokens input to the LLM, the influence caused by this difference will be marginal.}. For each configuration, we train a video MLLM and evaluate on the long video understanding benchmarks.


\paragraph{}

\setlength{\tabcolsep}{6pt} % 减小列间距
\begin{table}[h]
\caption{Experimental results under the same number of visual tokens.}
    \small
    \centering
    \begin{tabular}{ccccccccl}
    \toprule
\makecell[l]{\# Frames} & \makecell[c]{\#Tokens/\\Frames}&    \makecell[l]{\# Total\\Tokens}&\makecell[c]{Event-\\Bench}&  \makecell[c]{VNBench}& \makecell[c]{MLVU}&  \makecell[c]{LongVideo\\Bench} &\makecell[c]{VideoMME\\wo/w-subs}   &Avg.\\
    \midrule
        8 &729&    5832&18.33&  16.30&  50.98&  43.44& 46.22/53.67 &\\
        30&196&   5880&28.67& 31.11& 54.97&  48.90&53.19/60.19 &\\
        72&81&   5832&24.33& 37.56& 58.37&  \textbf{50.34}&53.04/61.11 &\\
        120&49&    5880&\underline{29.67}&  \underline{38.44}&  \underline{59.06}&  49.81&\underline{55.15}/\underline{61.67} &\\
        162&36&    5832&\textbf{33.00}&  \textbf{40.67}&  \textbf{62.83}&  \underline{50.04}&\textbf{55.19}/\textbf{62.00} &\\
     %    234&25&    5850&&  &  &  & &\\
     % 365& 16& 5840& & & & & &\\
     \bottomrule
    \end{tabular}
    \label{tab:same_token_result}
\end{table}


\paragraph{}






==> sec/old_table.tex <==
\begin{table}[h]
\caption{Experiment results on representative long video understanding benchmarks.}
    \small
    \centering
    \begin{tabular}{lcccccc}
    \toprule
\makecell[l]{Models}&  \makecell[c]{EventBench}&  \makecell[c]{VNBench}&  \makecell[c]{VideoMME\\wo/w-subs}& \makecell[c]{MLVU}&  \makecell[c]{LongVideoBench}&\makecell[c]{Avg.}\\
    \midrule
    \multicolumn{7}{c}{\textit{Proprietary MLLMs}}\\
    \midrule
        GPT-4o& 53.33 &  64.4&  71.90/77.20&  64.60& 66.7& \\
        Gemini-1.5-Pro&43.24 & 66.7& 75.00/81.30& & 64.0& \\
        GPT-4V&32.65 & 48.9& 59.90/63.30& 49.20& 59.1& \\
        Qwen-VL-Max& & & 51.3/51.2& 42.2& &\\
    \midrule
    \multicolumn{7}{c}{\textit{Open-Source MLLMs}}\\
        PLLaVA-13B& 33.15& & & & 45.6& \\
        Video-CCAM-14B&  &  &  53.2/57.4&  63.1& & \\
        VILA-1.5-34B&  &  &  62.3/64.1&  56.7& & \\
        ShareGPT4Video-8B&  &  &  39.9/43.6&  46.4& 39.7& \\
 IXC-2.5-7B& & & 55.8/-& 58.8& &\\
        Video-ChatGPT-7B& 11.78& 4.1& & 31.3& & \\
        Video-LLaVA-7B& 5.87& 12.4& 39.9/41.6& 47.3& & \\
        LLaMA-VID-long-7B&  0.04&  10.8&  &  33.2& & \\
        VideoLLaMA2-7B&  &  &  46.6/-&  48.5& & \\
        LongVA-7B&  &  &  52.6/-&  56.3& & \\
        % TimeChat-7B&  &  &  &  30.9& & \\
        MovieChat-7B& 16.21& & & 25.8& & \\
        VideoChat2-7B& 29.41& 12.4& 39.5/43.8& & & \\
        ST-LLM-7B&  37.71&  22.7&  37.9/42.3&  & & \\
 Kangaroo-7B& & & 56.0/57.6& 61.0& 54.8&\\
        xxx-7B (Ours)&  51.19&  40.37&  56.6/62.6&  62.2& 53.3& \\
    
    \bottomrule
    \end{tabular}
    \label{tab:main_exp}
\end{table}


% \begin{table}
%     \caption{Caption}
%     \centering
%     \begin{tabular}{lccccc}
%     \toprule
%          \multirow{2}{*}{Models}&  \multirow{2}{*}{\makecell[c]{Max\\Frames}}&  \multicolumn{4}{c}{Video Duration}\\
%          &  &  (8,15]&  (15,60]&  (180,600]& (900,3600]\\
%     \midrule
%          GPT-4o&256 & 71.6&76.8 &66.7 &61.6 \\
%          PLLaVA-34B& 16 & 60.1 & 66.8 & 50.8 & 49.1\\
%          Phi-3-Vision-Instruct& 16 & 58.3 & 59.6 & 48.4 & 45.1\\
%          Idefics2&  &  &  &  & \\
%          Mantis-Idefics2&  &  &  &  & \\
%          LLaVA-Next-Video&  &  &  &  & \\
%          xxx (Ours)&  &  &  &  & \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}

\begin{table}
    \centering
    \begin{tabular}{lccccc}
    \toprule
         Model&  Frames&  Short&  Medium&  Long& Overall\\
    \midrule
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
    \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{ccc}
         &  MLVU&  VideoMME\\
         LLaVA-OneVision&  64.70&  58.20/61.50\\
         ours&  62.83&  55.19/62.00\\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{ccc}
         Visual Context Length&  \# Visual Tokens& \# Frames\\
         6,000&  51& 118\\
         14,000&  78& 178\\
         30,000&  116& 258\\
         62,000&  169& 367\\
 126,000& 243&517\\
    \end{tabular}
    \caption{Estimated Optimal Visual Tokens and Frames for Various Visual Context Length.}
    \label{tab:configuration}
\end{table}
